Towards Optimal Prior-Free Permissionless Rebate Mechanisms, with applications to Automated Market Makers & Combinatorial Orderflow Auctions

Maximal Extractable Value (MEV) has become a critical issue for blockchain ecosystems, as it enables validators or block proposers to extract value by ordering, including or censoring users' transactions. This paper aims to present a formal approach for determining the appropriate compensation for users whose transactions are executed in bundles, as opposed to individually. We explore the impact of MEV on users, discuss the Shapley value as a solution for fair compensation, and delve into the mechanisms of MEV rebates and auctions as a means to undermine the power of the block producer.

==> notes.tex <==
Finish the auction section

In symmetric games add the simple case proof of Costs for completeness.

Finish our contributions

Add related work.

Discussion -> Funding public goods.

Add proves.

Prove opearator is GSP.

==> sections/axioms.tex <==



Maximal Extractable Value rebates or MEVR for short, are a type of incentive paid by builders to users who execute transactions that generate some surplus that the builder can extract. MEV rebates are paid out of the value generated by the transaction, and the amount of the rebate is typically determined by the MEV extracted by the builder and its paying policy.

Shapley values \cite{} are a mathematical concept used to allocate the total value generated by a group of players to each individual player in a cooperative game. The Shapley value of a player is based on the player's contribution to the total value generated by the group. In the context of MEV rebates, Shapley values seems a natural solution to be used to allocate the value generated by a transaction to the different participants involved in the block.

In this section, we will formalize the MEV rebates and different axioms that an ideal MEVR operator should have. 


To formalize MEV distribution and MEV rebates, we could use the notation introduced in \cite{mazorra2022price}. However, we can have more general definition. Let $\mathcal S$ be the set of states $\mathcal T$ the set of transactions and $\mathcal B=2^{\mathcal T}$ the set of bundles. Each player $i$ send a bundle $B_i$ to a "perfect MEV oracle". 
That is, the player can compute $\text{MEV}(\texttt{st},\mathcal P)$ where $\mathcal P=\{B_i\}_{i\in I}$. We will write $\text{MEV}$ as a map $v:\mathcal S\times 2^{\mathcal B}\rightarrow\mathbb R$. 
Observe that for a given state $\texttt{st}$ we can restrict $v$ to $\texttt{st}\times 2^{\mathcal B}$ and interpret this restriction as a \textit{coalitional form game} on a finite set of players $I$.

\textbf{Completness state-MEV}: Let $\mathcal P$ be a mempool, i.e. a set of bundles. For every monotonic map $v:2^{\mathcal P}\rightarrow \mathbb R$, there exist a valid state $\texttt{st}\in\mathcal S$ such that $\text{MEV}(\texttt{st},\cdot)_{|2^{\mathcal P}}=v(\cdot)$.

\begin{definition} A \textit{rebate value operator} or \textit{value} operator for short is a function that assigns each valuation $v:2^{N}\rightarrow \mathbb R$ to a vector of $(\phi_1,...,\phi_n)$ of $\mathbb R^n$. $\phi_i$ stands for the $i$'s payoff in the game, or alternatively for the measure of $i$'s contribution in the game.
\end{definition}

\textbf{Axiomatic characterization of value}: Now we will describe a set of desirable properties of an MEV rebate value operator. For a given set of bundles and state, we will denote by $v$ as the MEV function restricted to this state and sets.

\textbf{Efficency}: The players precisely distribute among themselves the value generated by their bundles. Namely,
\begin{equation*}
    \sum_{i\in N}\phi_i(v) = v(N)
\end{equation*}

Two players are said to be symmetric with respect to $v$ if their bundles make the same marginal contribution to any sub-mempool  i.e. for all $\mathcal P'\subseteq \{B_1,...,B_n\}$, it holds $v(\mathcal P'\cup\{B_i\})=v(\mathcal P'\cup\{B_j\})$ for all $B_i,B_j\not\in \mathcal P'$.

\textbf{Symmetry}: If bundles $B_i$ and $B_j$ are symmetric with respect to $v$, then $\phi_i(v)=\phi_j(v)$.
 
The next axiom requires that bundles that add zero MEV with respect to every other set of bundles have zero payoff.

\textbf{Zero-MEV bundles}: If a bundle is Zero-MEV with respect $v$, i.e. $v(\mathcal P'\cup i)=v(\mathcal P')$ for all $\mathcal P'\subseteq\mathcal P$, then $\phi_i(v)=0$.


For a bundle $B_i$ and a set of bundles $\mathcal P'\subseteq \mathcal P$, we define $D_i(v,\mathcal P')=v(\mathcal P'\cup B_i)-v(\mathcal P')$ as the $i'$ bundle contribution to the mempool $\mathcal P'$ with respect the value function $v$ (MEV over a state $\texttt{st}$).

\textbf{Strong monotonicity}: A value operator $\phi$ is strong monotonic if for every value functions $v,w$ such that $D_i(v,S)\geq D_i(w,S)$ for all $S\in 2^{\mathcal P}$.

\begin{theorem} Operator $\phi$ with these properties imply $\phi$ is Shapley values.
\end{theorem}

Another important property that can be strong against some deviations, players can generate "Sybil bundles". Any transaction can be splited with two or more transaction in a way that do not add any MEV separately but added in the mempool pairwise generate MEV. For example




Drawbacks:  Additionally, the complexity of the Shapley value calculation may make it challenging to implement in real-time blockchain systems.
%Shapley presented the value as an opeartor that assigns an expected marginal contribution to each player in the game with respect to a uniform distribution over the set of all permutations on the set of players.
\url{https://link.springer.com/article/10.1007/s10479-015-1859-8}

